Decoding Linguistic Representations of Human Brain

Language, as an information medium created by advanced organisms, has always been a concern of neuroscience regarding how it is represented in the brain. Decoding linguistic representations in the evoked brain has shown groundbreaking achievements, thanks to the rapid improvement of neuroimaging, medical technology, life sciences and artificial intelligence. In this work, we present a taxonomy of brain-to-language decoding of both textual and speech formats. This work integrates two types of research: neuroscience focusing on language understanding and deep learning-based brain decoding. Generating discernible language information from brain activity could not only help those with limited articulation, especially amyotrophic lateral sclerosis (ALS) patients but also open up a new way for the next generation's brain-computer interface (BCI). This article will help brain scientists and deep-learning researchers to gain a bird's eye view of fine-grained language perception, and thus facilitate their further investigation and research of neural process and language decoding.

==> figs/preserve.tex <==
\tikzstyle{my-box}=[
    rectangle,
    draw=hidden-draw,
    rounded corners,
    text opacity=1,
    minimum height=1.5em,
    minimum width=5em,
    inner sep=2pt,
    align=center,
    fill opacity=.5,
]
\tikzstyle{cause_leaf}=[my-box, minimum height=1.5em,
    fill=harvestgold!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]

\tikzstyle{class_leaf}=[my-box, minimum height=1.5em,
    fill=cyan!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]

\tikzstyle{detect_leaf}=[my-box, minimum height=1.5em,
    fill=cyan!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\tikzstyle{mitigate_leaf}=[my-box, minimum height=1.5em,
    fill=lightgreen!20, text=black, align=left,font=\scriptsize,
    inner xsep=2pt,
    inner ysep=4pt,
]
\begin{figure*}[tp]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{forest}
            forked edges,
            for tree={
                grow=east,
                reversed=true,
                anchor=base west,
                parent anchor=east,
                child anchor=west,
                base=left,
                font=\small,
                rectangle,
                draw=hidden-draw,
                rounded corners,
                align=left,
                minimum width=4em,
                edge+={darkgray, line width=1pt},
                s sep=3pt,
                inner xsep=2pt,
                inner ysep=3pt,
                ver/.style={rotate=90, child anchor=north, parent anchor=south, anchor=center},
            },
            where level=1{text width=5.8em,font=\scriptsize,}{},
            where level=2{text width=7.0em,font=\scriptsize,}{},
            where level=3{text width=8.8em,font=\scriptsize,}{},
            where level=4{text width=7.8em,font=\scriptsize,}{},
            [
                Linguistic Brain Decoding, ver, color=carminepink!100, fill=carminepink!15,
                text=black
                [
                    Brain-Network \\ Alignment , color=harvestgold!100, fill=harvestgold!100, text=black
                    [
                        Neural Tracking, color=harvestgold!100, fill=harvestgold!60,  text=black
                        [
                            Time Alignment, color=harvestgold!100, fill=harvestgold!40, text=black
                            	[
                            		Speech Flow, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{e.g. \citeauthor{ahissar2001speech}}
                                		, cause_leaf, text width=20em
                            		]
                            ]
                            [
                            		Uncertainty \\ Surprisal, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{e.g. \citeauthor{donhauser2020two,gillis2021neural}}
                                		, cause_leaf, text width=20em
                            		]
                            ] 
                            [
                            		Phoneme \& Word \\ Sequences, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{e.g. \citeauthor{brodbeck2018rapid, koskinen2020brain}}
                                		, cause_leaf, text width=20em
                            		]
                            ]
                        ]
                    ]
                    [
                        Neural Prediction, color=harvestgold!100, fill=harvestgold!60, text=black
                        [
                            Contextual Message, color=harvestgold!100, fill=harvestgold!40, text=black
                            [
                            		Single Neurons, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{e.g. \citeauthor{leonard2024large, khanna2024single}}
                                		, cause_leaf, text width=20em
                            		]
                            ]
                            [
                            		Cortical, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{e.g. \citeauthor{clark2013whatever, schrimpf2021neural,heilbron2022hierarchy}}
                                		, cause_leaf, text width=20em
                            		]
                            ]
                            [
                            		Artificial Networks, color=harvestgold!100, fill=harvestgold!20, text=black
                            		[
                                		{e.g. \citeauthor{ jain2020interpretable, caucheteux2021disentangling, toneva2022combining}}
                                		, cause_leaf, text width=20em
                            		]
                            ]
                        ]
                    ]
                ]
                [
                    Content \\ Classification , color=cyan!100, fill=cyan!100, text=black
                    [
                        Textual Stimuli, color=cyan!100, fill=cyan!60,  text=black
                        [
                           Word, color=cyan!100, fill=cyan!40, text=black
                            	[
                            		Classifiers, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{just2010neurosemantic, sudre2012tracking, anderson2017visually}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                            [
                            		Embedding Models, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{ e.g. \citeauthor{abnar2018experiential,pereira2018toward}}
                                		, class_leaf, text width=20em
                            		]
                            ] 
                        ]
                        [
                           Sentences, color=cyan!100, fill=cyan!40, text=black
                            	[
                            		Words Combine, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{anderson2017predicting, wang2017predicting, anderson2019integrated}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                            [
                            		Holistic Modeling, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{sun2019towards, gauthier2019linking}}
                                		, class_leaf, text width=20em
                            		]
                            ] 
                            [
                            		Semantic Models, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{jat2019relating,sun2020neural}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                            [
                            		Network Module, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{affolter2020brain2word, zou2021towards}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                        ]
                    ]
                    [
                        Speech Stimuli, color=cyan!100, fill=cyan!60, text=black
                        [
                            Semantics, color=cyan!100, fill=cyan!40, text=black
                            [
                            		Classifiers, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{liu2018speech, moses2019real}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                            [
                            		Network Module, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{bollens2022learning,defossez2023decoding}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                        ]
                        [
                            Speech Envelope, color=cyan!100, fill=cyan!40, text=black
                            [
                            		Signal Processing, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{vanthornhout2018speech}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                            [
                            		Network Module, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{crosse2016multivariate, accou2021modeling,thornton2022robust}\\ \citeauthor{xu2022decoding,accou2023decoding}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                            [
                            		Pre-trained Models, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{de2018decoding, zhu2023eeg2vec}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                            [
                            		Cock-tail Party, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{de2020machine}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                        ]
                        [
                            Mel-frequency \\ Cepstral Coefficient, color=cyan!100, fill=cyan!40, text=black
                            [
                            		Regression Models, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{krishna2019state, krishna2021advancing}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                            [
                            		Network Module, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{petrosyan2021compact}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                        ]
                        [
                            Speech Wave, color=cyan!100, fill=cyan!40, text=black
                            [
                            	Spectrogram, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{wang2020stimulus,guo2023end,senda2024auditory}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                            [
                            		Synthesizer \\ Parameters, color=cyan!100, fill=cyan!20, text=black
                            		[
                                		{e.g. \citeauthor{akbari2019towards}}
                                		, class_leaf, text width=20em
                            		]
                            ]
                        ]
                    ]
                ]
                [
                    Fine-grained \\ Recognition, color=lightgreen!100, fill=lightgreen!100, text=black
                    [
                        Brain Recording \\ Translation, color=lightgreen!100, fill=lightgreen!60, text=black
                        [
                            Network Module, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                            		Factuality Data \\ Enhancement, color=lightgreen!100, fill=lightgreen!20, text=black
                            		[
                                		{e.g. \citeauthor{makin2020machine}}
                                , mitigate_leaf, text width=20em
                            		]
                            ]
                        ]
                        [
                            Pre-trained Language \\ Models, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                            	BART, color=lightgreen!100, fill=lightgreen!20, text=black
                            		[
                                		{e.g. \citeauthor{wang2022open, xi2023unicorn,duan2023dewave, feng2023aligning}}
                                , mitigate_leaf, text width=20em
                            		]
                            ]
                            [
                            		GPT, color=lightgreen!100, fill=lightgreen!20, text=black
                            		[
                                		{e.g. \citeauthor{tang2023semantic, chen2024openvocabulary}}
                                , mitigate_leaf, text width=20em
                            		]
                            ]
                            [
                            		Llama, color=lightgreen!100, fill=lightgreen!20, text=black
                            		[
                                		{e.g. \citeauthor{antonello2024many}}
                                , mitigate_leaf, text width=20em
                            		]
                            ]
                        ]
                        [
                            Pre-trained Speech \\ Models, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                                Whisper, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                		{e.g. \citeauthor{yang2024decode}}
                                , mitigate_leaf, text width=20em
                                ]
                            ]
                        ]
                    ]
                    [
                        Speech \\ Neuroprosthesis, color=lightgreen!100, fill=lightgreen!60, text=black
                        [
                               Phoneme, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                                Instance-based \\ Matching, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g. \citeauthor{suppes1997brain, suppes1998brain, d2009toward}}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                            [
                                Classifiers, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g. Linear classifier: \citeauthor{tankus2012structured} \\
                                    SVM: \citeauthor{dasalla2009single, wang2013analysis, stavisky2018decoding} \\
                                    naive Bayes classifier: \citeauthor{pei2011decoding} \\...}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                            [
                               Dimensionality \\ Reduction, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g. PCA: \citeauthor{kellis2010decoding} \hspace{2mm} FDA: \citeauthor{brumberg2011classification} \\
                                    LDA: \citeauthor{deng2010eeg, kim2014eeg,mugler2014direct} \\...}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                        ]
                        [
                           Modest Vocabulary, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                                Classifiers, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g.  \citeauthor{mohanchandra2016communication,martin2016word}\\ \citeauthor{nguyen2017inferring,gonzalez2017sonification}}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                            [
                                Network Module, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g. \citeauthor{salama2014recognition,zhao2015classifying}\\
                                    \citeauthor{saha2019hierarchical,dash2020decoding,petrosyan2021compact}}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                        ]
                        [
                           Open Vocabulary, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                                Hybrid System, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g. Gaussian-based: \citeauthor{herff2015brain,moses2016neural}\\
                                    NN-based: \citeauthor{willett2023high, metzger2023high}}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                            [
                                End-to-End System, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g. \citeauthor{feng2024endtoend,yuan2024improving}}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                        ]
                        [
                           Brain-to-Speech, color=lightgreen!100, fill=lightgreen!40, text=black
                            [
                               Non-deep Learning, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g. \citeauthor{herff2019generating}}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                            [
                                Speech Properties, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g. \citeauthor{guenther2009wireless, angrick2019speech, chen2024neural}}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                            [
                               Synthesizer \\ Parameters, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g. \citeauthor{guenther2009wireless, chen2024neural}}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                            [
                               Articulators, color=lightgreen!100, fill=lightgreen!20, text=black
                                [
                                    {e.g. \citeauthor{bouchard2013functional,bocquelet2014robust}}
                                    , mitigate_leaf, text width=20em
                                ]
                            ]
                        ]
                    ]
                ]
           ]
        \end{forest}
    }
    \caption{The main content flow and categorization of this survey.}
    \label{categorization_of_survey}
\end{figure*}

==> sn-example.tex <==


\section{Results}\label{sec2}

\subsection{Text evaluation}\label{subsec2.1}

Decoding verbal stimuli from brain responses is a fundamental task, which has profound implications for studying brain perception paradigms. A scientific evaluation indicator quantifies the similarity between decoded text and stimulus text, which the fields of machine translation and speech recognition can inspire.

\begin{itemize}
    \item BLUE: BLEU (Bilingual Evaluation Understudy) \cite{papineni2002bleu} is a metric used for evaluating the quality of machine-translated text from one language to another, which has become a standard measure for assessing the semantic similarity between text in two languages. BLEU calculates the precision of n-grams compared to reference translations, typically including unigrams, bigrams, trigrams, and 4-grams. To prevent the unfair reward for over-generating common words, BLEU uses clipping, which limits the count of each n-gram to the maximum count observed in any single reference translation. BLEU includes a brevity penalty to address the preference for shorter translations. In brain decoding, BLUE is usually used in more difficult scenarios, such as sequential decoding of non-invasive recordings. The accurate textual information is typically unavailable to generate due to the data quality while the semantic-related representations are of great significance. The calculation process is as follows, where $c$ is the length of the machine translation, $r$ is the effective reference length, $w_n$ are weights assigned to different n-gram lengths, and $p_n$ are the n-gram precisions.

\begin{equation}
\text{BP} = 
\begin{cases} 
1 & \text{if } c > r \\
e^{(1 - \frac{r}{c})} & \text{if } c \leq r 
\end{cases}
\end{equation}    
\begin{equation}
\text{BLEU} = \text{BP} \cdot \exp \left( \sum_{n=1}^{N} w_n \log p_n \right)
\end{equation}  


    \item ROUGE: ROUGE (Recall-Oriented Understudy for Gisting Evaluation) \cite{lin2004rouge} is a set of metrics used for evaluating automatic text summarization and machine translation systems. Unlike BLUE, it focuses more on recall, which is defined as the number of overlapping between the generated and reference texts divided by the total n-grams in the reference texts. ROUGE includes several variants focusing on different aspects of the generated text, among which ROUGE-N is widely adopted in brain decoding tasks. It measures n-gram overlap between the generated text and reference texts, and unigram is the most common ($N=1$). The calculation process is as follows, where $Count_{match}(gram_n)$ is the number of n-grams in both the generated and reference texts.
    
\begin{equation}
\text{ROUGE-N} = \frac{\sum_{S \in \{\text{Reference Summaries}\}} \sum_{gram_n \in S} \text{Count}_{match}(gram_n)}{\sum_{S \in \{\text{Reference Summaries}\}} \sum_{gram_n \in S} \text{Count}(gram_n)}
\end{equation}  

    \item BERTScore: BERTScore \cite{zhang2019bertscore} is a recent metric for evaluating the quality of the generated text. Unlike BLEU and ROUGE, BERTScore leverages deep contextualized embeddings from BERT to capture semantic similarity between the generated and the reference text. Instead of matching exact n-grams, BERTScore matches tokens based on their semantic similarity as represented by BERT embeddings. It computes precision, recall, and F1 scores based on the cosine similarity between the embeddings of tokens in the generated text and reference text. The calculation process is as follows, where $\hat{x}$ is the decoding candidate and $x$ is the corresponding reference.

\begin{equation}
R = \frac{1}{|x|} \sum_{x_i \in x} \max_{\hat{x}_j \in \hat{x}} x_i^\top \hat{x}_j \hspace{5mm}
P = \frac{1}{|\hat{x}|} \sum_{\hat{x}_i \in \hat{x}} \max_{x_j \in x} x_j^\top \hat{x}_i \hspace{5mm}
F_{\text{BERT}} = 2 \frac{P \cdot R}{P + R}
\end{equation}  


    \item WER: WER (word error rate) is a common metric used to evaluate the performance of ASR systems. It measures the accuracy of decoded hypotheses compared to reference transcriptions. For brain decoding, WER is widely adopted for speech neuroprosthesis, which aims to decode the inner speech of subjects without making distinguishable sounds given the invasive evoked brain recordings. It provides a straightforward, quantitative measure of how many errors are present in the generated text. In addition to the calculation on word level, CER (character word error rate) and PER (phoneme error rate) are carried out on character- and phoneme-level respectively. The calculation process of WER is as follows, where S, I and D stands for the number of substitution, insertion and deletion errors in the decoded sentences, and N stands for the total length of the reference transcription. 

\begin{equation}
WER = \frac{S+I+D}{N}
\end{equation}  
    
\end{itemize}


\subsection{Speech evaluation}\label{subsec2.2}

\begin{itemize}
    \item PCC: PCC (Pearson correlation coefficient) is a measure of the linear relationship between two continuous variables. It quantifies the degree to which the variables are linearly related, indicating both the strength and direction of the relationship. Considering the difficulty of directly synthesizing speech waves, PCC is widely used to evaluate the correlation between the synthesized speech and the reference. The formula for calculating the Pearson Correlation Coefficient between two variables $X=(X_1,...,X_n)$ and $Y=(Y_1,...,Y_n)$ is as follows.

\begin{equation}
    r = \frac{\sum_{i=1}^{n} (X_i - \overline{X})(Y_i - \overline{Y})}{\sqrt{\sum_{i=1}^{n} (X_i - \overline{X})^2} \sqrt{\sum_{i=1}^{n} (Y_i - \overline{Y})^2}}
\end{equation}
    \item STOI: STOI (Short-Time Objective Intelligibility) is a metric used for evaluating the intelligibility of speech signals. It is designed to provide an objective measure that correlates well with human subjective intelligibility ratings. As for synthesizing speech from evoked brain activities, STOI is adopted to evaluate the intelligibility of the reconstructed speech waveform.
    
    \item FFE: FFE (F0 frame error) is a metric used to evaluate the accuracy of pitch (fundamental frequency, F0) tracking systems, particularly in the context of speech synthesis. It measures the percentage of frames in which the estimated F0 value is incorrect compared to a reference. 

    
    \item MCD: MCD (mel-cepstral distortion) is a metric used to evaluate the performance of speech synthesis systems. It measures the difference between the MFCCs of the synthesized speech and the reference speech based on the Euclidean distance. The calculation process is as follows, where $M$ and $T$ are the numbers of MFCCs and frames respectively.

\begin{equation}
    d_t = \sqrt{ \sum_{m=1}^{M} \left( c_{t, m}^{\text{ref}} - c_{t, m}^{\text{syn}} \right)^2 } \hspace{5mm} \text{MCD} = \frac{10}{\ln(10)} \sqrt{2} \cdot \frac{1}{T} \sum_{t=1}^{T} d_t
\end{equation}

    \item MOS: MOS (mean opinion score) is a widely used metric for evaluating the perceived quality of audio, video, and multimedia content. It is particularly prevalent in the fields of speech synthesis, speech enhancement, and telecommunication systems. MOS provides a subjective measure of quality based on human judgments, making it a crucial tool for assessing user experience. Typically, MOS uses a five-point scale where participants rate the quality of the content, with 1 being the lowest quality and 5 being the highest. MOS is generated by calculating the mean of all ratings. It is conceivable that MOS evaluation has certain requirements for synthesis speech. It may be difficult for manual subjective evaluation to distinguish the difference when the synthesis quality is poor.

\end{itemize}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\section{This is an example for first level head---section head}\label{sec3}

%\subsection{This is an example for second level head---subsection head}\label{subsec2}

\subsubsection{This is an example for third level head---subsubsection head}\label{subsubsec2}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. 

\section{Equations}\label{sec4}

Equations in \LaTeX\ can either be inline or on-a-line by itself (``display equations''). For
inline equations use the \verb+$...$+ commands. E.g.: The equation
$H\psi = E \psi$ is written via the command \verb+$H \psi = E \psi$+.

For display equations (with auto generated equation numbers)
one can use the equation or align environments:
\begin{equation}
\|\tilde{X}(k)\|^2 \leq\frac{\sum\limits_{i=1}^{p}\left\|\tilde{Y}_i(k)\right\|^2+\sum\limits_{j=1}^{q}\left\|\tilde{Z}_j(k)\right\|^2 }{p+q}.\label{eq1}
\end{equation}
where,
\begin{align}
D_\mu &=  \partial_\mu - ig \frac{\lambda^a}{2} A^a_\mu \nonumber \\
F^a_{\mu\nu} &= \partial_\mu A^a_\nu - \partial_\nu A^a_\mu + g f^{abc} A^b_\mu A^a_\nu \label{eq2}
\end{align}
Notice the use of \verb+\nonumber+ in the align environment at the end
of each line, except the last, so as not to produce equation numbers on
lines where no equation numbers are required. The \verb+\label{}+ command
should only be used at the last line of an align environment where
\verb+\nonumber+ is not used.
\begin{equation}
Y_\infty = \left( \frac{m}{\textrm{GeV}} \right)^{-3}
    \left[ 1 + \frac{3 \ln(m/\textrm{GeV})}{15}
    + \frac{\ln(c_2/5)}{15} \right]
\end{equation}
The class file also supports the use of \verb+\mathbb{}+, \verb+\mathscr{}+ and
\verb+\mathcal{}+ commands. As such \verb+\mathbb{R}+, \verb+\mathscr{R}+
and \verb+\mathcal{R}+ produces $\mathbb{R}$, $\mathscr{R}$ and $\mathcal{R}$
respectively (refer Subsubsection~\ref{subsubsec2}).

\section{Tables}\label{sec5}

Tables can be inserted via the normal table and tabular environment. To put
footnotes inside tables you should use \verb+\footnotetext[]{...}+ tag.
The footnote appears just below the table itself (refer Tables~\ref{tab1} and \ref{tab2}). 
For the corresponding footnotemark use \verb+\footnotemark[...]+

\begin{table}[h]
\caption{Caption text}\label{tab1}%
\begin{tabular}{@{}llll@{}}
\toprule
Column 1 & Column 2  & Column 3 & Column 4\\
\midrule
row 1    & data 1   & data 2  & data 3  \\
row 2    & data 4   & data 5\footnotemark[1]  & data 6  \\
row 3    & data 7   & data 8  & data 9\footnotemark[2]  \\
\botrule
\end{tabular}
\footnotetext{Source: This is an example of table footnote. This is an example of table footnote.}
\footnotetext[1]{Example for a first table footnote. This is an example of table footnote.}
\footnotetext[2]{Example for a second table footnote. This is an example of table footnote.}
\end{table}

\noindent
The input format for the above table is as follows:

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. Please ignore this.       %%
%%=============================================%%
\bigskip
\begin{verbatim}
\begin{table}[<placement-specifier>]
\caption{<table-caption>}\label{<table-label>}%
\begin{tabular}{@{}llll@{}}
\toprule
Column 1 & Column 2 & Column 3 & Column 4\\
\midrule
row 1 & data 1 & data 2	 & data 3 \\
row 2 & data 4 & data 5\footnotemark[1] & data 6 \\
row 3 & data 7 & data 8	 & data 9\footnotemark[2]\\
\botrule
\end{tabular}
\footnotetext{Source: This is an example of table footnote. 
This is an example of table footnote.}
\footnotetext[1]{Example for a first table footnote.
This is an example of table footnote.}
\footnotetext[2]{Example for a second table footnote. 
This is an example of table footnote.}
\end{table}
\end{verbatim}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. Please ignore this.       %%
%%=============================================%%

\begin{table}[h]
\caption{Example of a lengthy table which is set to full textwidth}\label{tab2}
\begin{tabular*}{\textwidth}{@{\extracolsep\fill}lcccccc}
\toprule%
& \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]} & \multicolumn{3}{@{}c@{}}{Element 2\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%
Project & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ \\
\midrule
Element 3  & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$\\
Element 4  & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$\\
\botrule
\end{tabular*}
\footnotetext{Note: This is an example of table footnote. This is an example of table footnote this is an example of table footnote this is an example of~table footnote this is an example of table footnote.}
\footnotetext[1]{Example for a first table footnote.}
\footnotetext[2]{Example for a second table footnote.}
\end{table}

In case of double column layout, tables which do not fit in single column width should be set to full text width. For this, you need to use \verb+\begin{table*}+ \verb+...+ \verb+\end{table*}+ instead of \verb+\begin{table}+ \verb+...+ \verb+\end{table}+ environment. Lengthy tables which do not fit in textwidth should be set as rotated table. For this, you need to use \verb+\begin{sidewaystable}+ \verb+...+ \verb+\end{sidewaystable}+ instead of \verb+\begin{table*}+ \verb+...+ \verb+\end{table*}+ environment. This environment puts tables rotated to single column width. For tables rotated to double column width, use \verb+\begin{sidewaystable*}+ \verb+...+ \verb+\end{sidewaystable*}+.

\begin{sidewaystable}
\caption{Tables which are too long to fit, should be written using the ``sidewaystable'' environment as shown here}\label{tab3}
\begin{tabular*}{\textheight}{@{\extracolsep\fill}lcccccc}
\toprule%
& \multicolumn{3}{@{}c@{}}{Element 1\footnotemark[1]}& \multicolumn{3}{@{}c@{}}{Element\footnotemark[2]} \\\cmidrule{2-4}\cmidrule{5-7}%
Projectile & Energy	& $\sigma_{calc}$ & $\sigma_{expt}$ & Energy & $\sigma_{calc}$ & $\sigma_{expt}$ \\
\midrule
Element 3 & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$ \\
Element 4 & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$ \\
Element 5 & 990 A & 1168 & $1547\pm12$ & 780 A & 1166 & $1239\pm100$ \\
Element 6 & 500 A & 961  & $922\pm10$  & 900 A & 1268 & $1092\pm40$ \\
\botrule
\end{tabular*}
\footnotetext{Note: This is an example of table footnote this is an example of table footnote this is an example of table footnote this is an example of~table footnote this is an example of table footnote.}
\footnotetext[1]{This is an example of table footnote.}
\end{sidewaystable}

\section{Figures}\label{sec6}

As per the \LaTeX\ standards you need to use eps images for \LaTeX\ compilation and \verb+pdf/jpg/png+ images for \verb+PDFLaTeX+ compilation. This is one of the major difference between \LaTeX\ and \verb+PDFLaTeX+. Each image should be from a single input .eps/vector image file. Avoid using subfigures. The command for inserting images for \LaTeX\ and \verb+PDFLaTeX+ can be generalized. The package used to insert images in \verb+LaTeX/PDFLaTeX+ is the graphicx package. Figures can be inserted via the normal figure environment as shown in the below example:

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. Please ignore this.       %%
%%=============================================%%
\bigskip
\begin{verbatim}
\begin{figure}[<placement-specifier>]
\centering
\includegraphics{<eps-file>}
\caption{<figure-caption>}\label{<figure-label>}
\end{figure}
\end{verbatim}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. Please ignore this.       %%
%%=============================================%%

\begin{figure}[h]
\centering
\includegraphics[width=0.9\textwidth]{fig.eps}
\caption{This is a widefig. This is an example of long caption this is an example of long caption  this is an example of long caption this is an example of long caption}\label{fig1}
\end{figure}

In case of double column layout, the above format puts figure captions/images to single column width. To get spanned images, we need to provide \verb+\begin{figure*}+ \verb+...+ \verb+\end{figure*}+.

For sample purpose, we have included the width of images in the optional argument of \verb+\includegraphics+ tag. Please ignore this. 

\section{Algorithms, Program codes and Listings}\label{sec7}

Packages \verb+algorithm+, \verb+algorithmicx+ and \verb+algpseudocode+ are used for setting algorithms in \LaTeX\ using the format:

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. Please ignore this.       %%
%%=============================================%%
\bigskip
\begin{verbatim}
\begin{algorithm}
\caption{<alg-caption>}\label{<alg-label>}
\begin{algorithmic}[1]
. . .
\end{algorithmic}
\end{algorithm}
\end{verbatim}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. Please ignore this.       %%
%%=============================================%%

You may refer above listed package documentations for more details before setting \verb+algorithm+ environment. For program codes, the ``verbatim'' package is required and the command to be used is \verb+\begin{verbatim}+ \verb+...+ \verb+\end{verbatim}+. 

Similarly, for \verb+listings+, use the \verb+listings+ package. \verb+\begin{lstlisting}+ \verb+...+ \verb+\end{lstlisting}+ is used to set environments similar to \verb+verbatim+ environment. Refer to the \verb+lstlisting+ package documentation for more details.

A fast exponentiation procedure:

\lstset{texcl=true,basicstyle=\small\sf,commentstyle=\small\rm,mathescape=true,escapeinside={(*}{*)}}
\begin{lstlisting}
begin
  for $i:=1$ to $10$ step $1$ do
      expt($2,i$);  
      newline() od                (*\textrm{Comments will be set flush to the right margin}*)
where
proc expt($x,n$) $\equiv$
  $z:=1$;
  do if $n=0$ then exit fi;
     do if odd($n$) then exit fi;                 
        comment: (*\textrm{This is a comment statement;}*)
        $n:=n/2$; $x:=x*x$ od;
     { $n>0$ };
     $n:=n-1$; $z:=z*x$ od;
  print($z$). 
end
\end{lstlisting}

\begin{algorithm}
\caption{Calculate $y = x^n$}\label{algo1}
\begin{algorithmic}[1]
\Require $n \geq 0 \vee x \neq 0$
\Ensure $y = x^n$ 
\State $y \Leftarrow 1$
\If{$n < 0$}\label{algln2}
        \State $X \Leftarrow 1 / x$
        \State $N \Leftarrow -n$
\Else
        \State $X \Leftarrow x$
        \State $N \Leftarrow n$
\EndIf
\While{$N \neq 0$}
        \If{$N$ is even}
            \State $X \Leftarrow X \times X$
            \State $N \Leftarrow N / 2$
        \Else[$N$ is odd]
            \State $y \Leftarrow y \times X$
            \State $N \Leftarrow N - 1$
        \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. Please ignore this.       %%
%%=============================================%%
\bigskip
\begin{minipage}{\hsize}%
\lstset{frame=single,framexleftmargin=-1pt,framexrightmargin=-17pt,framesep=12pt,linewidth=0.98\textwidth,language=pascal}% Set your language (you can change the language for each code-block optionally)
%%% Start your code-block
\begin{lstlisting}
for i:=maxint to 0 do
begin
{ do nothing }
end;
Write('Case insensitive ');
Write('Pascal keywords.');
\end{lstlisting}
\end{minipage}

\section{Cross referencing}\label{sec8}

Environments such as figure, table, equation and align can have a label
declared via the \verb+\label{#label}+ command. For figures and table
environments use the \verb+\label{}+ command inside or just
below the \verb+\caption{}+ command. You can then use the
\verb+\ref{#label}+ command to cross-reference them. As an example, consider
the label declared for Figure~\ref{fig1} which is
\verb+\label{fig1}+. To cross-reference it, use the command 
\verb+Figure \ref{fig1}+, for which it comes up as
``Figure~\ref{fig1}''. 

To reference line numbers in an algorithm, consider the label declared for the line number 2 of Algorithm~\ref{algo1} is \verb+\label{algln2}+. To cross-reference it, use the command \verb+\ref{algln2}+ for which it comes up as line~\ref{algln2} of Algorithm~\ref{algo1}.

\subsection{Details on reference citations}\label{subsec7}

Standard \LaTeX\ permits only numerical citations. To support both numerical and author-year citations this template uses \verb+natbib+ \LaTeX\ package. For style guidance please refer to the template user manual.

Here is an example for \verb+\cite{...}+: \cite{bib1}. Another example for \verb+\citep{...}+: \citep{bib2}. For author-year citation mode, \verb+\cite{...}+ prints Jones et al. (1990) and \verb+\citep{...}+ prints (Jones et al., 1990).

All cited bib entries are printed at the end of this article: \cite{bib3}, \cite{bib4}, \cite{bib5}, \cite{bib6}, \cite{bib7}, \cite{bib8}, \cite{bib9}, \cite{bib10}, \cite{bib11}, \cite{bib12} and \cite{bib13}.


\section{Examples for theorem like environments}\label{sec10}

For theorem like environments, we require \verb+amsthm+ package. There are three types of predefined theorem styles exists---\verb+thmstyleone+, \verb+thmstyletwo+ and \verb+thmstylethree+ 

%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. Please ignore this.       %%
%%=============================================%%
\bigskip
\begin{tabular}{|l|p{19pc}|}
\hline
\verb+thmstyleone+ & Numbered, theorem head in bold font and theorem text in italic style \\\hline
\verb+thmstyletwo+ & Numbered, theorem head in roman font and theorem text in italic style \\\hline
\verb+thmstylethree+ & Numbered, theorem head in bold font and theorem text in roman style \\\hline
\end{tabular}
\bigskip
%%=============================================%%
%% For presentation purpose, we have included  %%
%% \bigskip command. Please ignore this.       %%
%%=============================================%%

For mathematics journals, theorem styles can be included as shown in the following examples:

\begin{theorem}[Theorem subhead]\label{thm1}
Example theorem text. Example theorem text. Example theorem text. Example theorem text. Example theorem text. 
Example theorem text. Example theorem text. Example theorem text. Example theorem text. Example theorem text. 
Example theorem text. 
\end{theorem}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\begin{proposition}
Example proposition text. Example proposition text. Example proposition text. Example proposition text. Example proposition text. 
Example proposition text. Example proposition text. Example proposition text. Example proposition text. Example proposition text. 
\end{proposition}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\begin{example}
Phasellus adipiscing semper elit. Proin fermentum massa
ac quam. Sed diam turpis, molestie vitae, placerat a, molestie nec, leo. Maecenas lacinia. Nam ipsum ligula, eleifend
at, accumsan nec, suscipit a, ipsum. Morbi blandit ligula feugiat magna. Nunc eleifend consequat lorem. 
\end{example}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\begin{remark}
Phasellus adipiscing semper elit. Proin fermentum massa
ac quam. Sed diam turpis, molestie vitae, placerat a, molestie nec, leo. Maecenas lacinia. Nam ipsum ligula, eleifend
at, accumsan nec, suscipit a, ipsum. Morbi blandit ligula feugiat magna. Nunc eleifend consequat lorem. 
\end{remark}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\begin{definition}[Definition sub head]
Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. Example definition text. 
\end{definition}

Additionally a predefined ``proof'' environment is available: \verb+\begin{proof}+ \verb+...+ \verb+\end{proof}+. This prints a ``Proof'' head in italic font style and the ``body text'' in roman font style with an open square at the end of each proof environment. 

\begin{proof}
Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. 
\end{proof}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text. Sample body text.

\begin{proof}[Proof of Theorem~{\upshape\ref{thm1}}]
Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. Example for proof text. 
\end{proof}

\noindent
For a quote environment, use \verb+\begin{quote}...\end{quote}+
\begin{quote}
Quoted text example. Aliquam porttitor quam a lacus. Praesent vel arcu ut tortor cursus volutpat. In vitae pede quis diam bibendum placerat. Fusce elementum
convallis neque. Sed dolor orci, scelerisque ac, dapibus nec, ultricies ut, mi. Duis nec dui quis leo sagittis commodo.
\end{quote}

Sample body text. Sample body text. Sample body text. Sample body text. Sample body text (refer Figure~\ref{fig1}). Sample body text. Sample body text. Sample body text (refer Table~\ref{tab3}). 

\section{Methods}\label{sec11}

Topical subheadings are allowed. Authors must ensure that their Methods section includes adequate experimental and characterization data necessary for others in the field to reproduce their work. Authors are encouraged to include RIIDs where appropriate. 

\textbf{Ethical approval declarations} (only required where applicable) Any article reporting experiment/s carried out on (i)~live vertebrate (or higher invertebrates), (ii)~humans or (iii)~human samples must include an unambiguous statement within the methods section that meets the following requirements: 

\begin{enumerate}[1.]
\item Approval: a statement which confirms that all experimental protocols were approved by a named institutional and/or licensing committee. Please identify the approving body in the methods section

\item Accordance: a statement explicitly saying that the methods were carried out in accordance with the relevant guidelines and regulations

\item Informed consent (for experiments involving humans or human tissue samples): include a statement confirming that informed consent was obtained from all participants and/or their legal guardian/s
\end{enumerate}

If your manuscript includes potentially identifying patient/participant information, or if it describes human transplantation research, or if it reports results of a clinical trial then  additional information will be required. Please visit (\url{https://www.nature.com/nature-research/editorial-policies}) for Nature Portfolio journals, (\url{https://www.springer.com/gp/authors-editors/journal-author/journal-author-helpdesk/publishing-ethics/14214}) for Springer Nature journals, or (\url{https://www.biomedcentral.com/getpublished/editorial-policies\#ethics+and+consent}) for BMC.

\section{Discussion}\label{sec12}

Discussions should be brief and focused. In some disciplines use of Discussion or `Conclusion' is interchangeable. It is not mandatory to use both. Some journals prefer a section `Results and Discussion' followed by a section `Conclusion'. Please refer to Journal-level guidance for any specific requirements. 

\section{Conclusion}\label{sec13}

Conclusions may be used to restate your hypothesis or research question, restate your major findings, explain the relevance and the added value of your work, highlight any limitations of your study, describe future directions for research and recommendations. 

In some disciplines use of Discussion or 'Conclusion' is interchangeable. It is not mandatory to use both. Please refer to Journal-level guidance for any specific requirements. 

\backmatter

\bmhead{Supplementary information}

If your article has accompanying supplementary file/s please state so here. 

Authors reporting data from electrophoretic gels and blots should supply the full unprocessed scans for key as part of their Supplementary information. This may be requested by the editorial team/s if it is missing.

Please refer to Journal-level guidance for any specific requirements.

\bmhead{Acknowledgements}

Acknowledgements are not compulsory. Where included they should be brief. Grant or contribution numbers may be acknowledged.

Please refer to Journal-level guidance for any specific requirements.

\section*{Declarations}

Some journals require declarations to be submitted in a standardised format. Please check the Instructions for Authors of the journal to which you are submitting to see if you need to complete this section. If yes, your manuscript must contain the following sections under the heading `Declarations':

\begin{itemize}
\item Funding
\item Conflict of interest/Competing interests (check journal-specific guidelines for which heading to use)
\item Ethics approval and consent to participate
\item Consent for publication
\item Data availability 
\item Materials availability
\item Code availability 
\item Author contribution
\end{itemize}

\noindent
If any of the sections are not relevant to your manuscript, please include the heading and write `Not applicable' for that section. 

%%===================================================%%
%% For presentation purpose, we have included        %%
%% \bigskip command. Please ignore this.             %%
%%===================================================%%
\bigskip
\begin{flushleft}%
Editorial Policies for:

\bigskip\noindent
Springer journals and proceedings: \url{https://www.springer.com/gp/editorial-policies}

\bigskip\noindent
Nature Portfolio journals: \url{https://www.nature.com/nature-research/editorial-policies}

\bigskip\noindent
\textit{Scientific Reports}: \url{https://www.nature.com/srep/journal-policies/editorial-policies}

\bigskip\noindent
BMC journals: \url{https://www.biomedcentral.com/getpublished/editorial-policies}
\end{flushleft}

\begin{appendices}

\section{Section title of first appendix}\label{secA1}

An appendix contains supplementary information that is not an essential part of the text itself but which may be helpful in providing a more comprehensive understanding of the research problem or it is information that is too cumbersome to be included in the body of the paper.

%%=============================================%%
%% For submissions to Nature Portfolio Journals %%
%% please use the heading ``Extended Data''.   %%
%%=============================================%%

%%=============================================================%%
%% Sample for another appendix section			       %%
%%=============================================================%%

%% \section{Example of another appendix section}\label{secA2}%
%% Appendices may be used for helpful, supporting or essential material that would otherwise 
%% clutter, break up or be distracting to the text. Appendices can consist of sections, figures, 
%% tables and equations etc.

\end{appendices}

==> test.tex <==
\begin{table}[t!]
\caption{Representative datasets for linguistic sequence decoding of brain recordings. We annotate with the main author’s information for datasets without names.}
\begin{adjustbox}{center}
\centering
\label{Dataset}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Dataset & Language & Type & Experiment & Subjects & Vocabulary & Sentences & Task \\ \hline
ZuCo \cite{hollenstein2018zuco} & Eng & EEG & NR & 12 & - & 300 & BRT \\ \hline
\end{tabular}
\end{adjustbox}
\end{table}
